Distributed In-Context Learning under Non-IID Among Clients

Advancements in large language models (LLMs) have shown their effectiveness in multiple complicated natural language reasoning tasks. A key challenge remains in adapting these models efficiently to new or unfamiliar tasks. In-context learning (ICL) provides a promising solution for few-shot adaptation by retrieving a set of data points relevant to a query, called in-context examples (ICE), from a training dataset and providing them during the inference as context. Most existing studies utilize a centralized training dataset, yet many real-world datasets may be distributed among multiple clients, and remote data retrieval can be associated with costs. Especially when the client data are non-identical independent distributions (non-IID), retrieving from clients a proper set of ICEs needed for a test query presents critical challenges. In this paper, we first show that in this challenging setting, test queries will have different preferences among clients because of non-IIDness, and equal contribution often leads to suboptimal performance. We then introduce a novel approach to tackle the distributed non-IID ICL problem when a data usage budget is present. The principle is that each client's proper contribution (budget) should be designed according to the preference of each query for that client. Our approach uses a data-driven manner to allocate a budget for each client, tailored to each test query. Through extensive empirical studies on diverse datasets, our framework demonstrates superior performance relative to competing baselines.

==> misc/alg_train_ba.tex <==
\begin{algorithm}
\caption{Train Budget Allocator for client $c$}
\label{alg:train_ba}
\begin{algorithmic}[1]
    \REQUIRE Initialized $c^{\text{th}}$ Classifier $f_c(e;\theta_c)$, Dataset $\mc{D}_{\text{proxy}}^{c}$, Training iteration $T$\\
    \hfill\textcolor{Skyblue}{\textbf{\underline{/* Training for $c^\text{th}$ client */}}}\hfill \mbox{} \\
    \FOR{$1\ldots t \ldots T$}
       \STATE $\theta_c \leftarrow \theta_c - \nabla_{\theta_c} \frac{1}{|D|} \sum_{D}\mc{L}_{\text{CE}} (f_c(e_j;\theta_c), B_j)$ \\
       \hfill where $D =\{(e_j, B_j)\}_{j=1}^{|D|} \subset \mc{D}_{\text{proxy}}^{c}$
    \ENDFOR
    \RETURN $f_c(e;\theta_c)$
\end{algorithmic}
\end{algorithm}

==> misc/tab_main_old.tex <==
\begin{table*}[t]
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{ccccccccccccc}
    \thickhline
        \multicolumn{3}{c}{\multirow{2}{*}{Algorithm}} & \multicolumn{8}{c}{Dataset}  &&\multirow{2}{*}{Avg}\\\cmidrule{4-11} 
        & && SST-5 & Amazon & Yelp & CR & MR & Yahoo & Agnews & Subj &&  \\\hline 
        \multirow{11}{*}{\begin{sideways}Original\end{sideways}} & Zero-shot 
                     && 29.19 & 24.70 & 31.23 
                     & 62.07 & 73.95 & 25.87 & 67.60 & 50.55 && 45.64\\
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Proxy-only-train 
                     && 38.86{\tiny $\pm$ 1.66} & 18.70{\tiny $\pm$ 0.07} 
                     & 20.55{\tiny $\pm$ 0.04} & 62.56{\tiny $\pm$ 0.93} 
                     & 70.75{\tiny $\pm$ 1.47} & 11.54{\tiny $\pm$ 0.84} & 82.03{\tiny $\pm$ 0.62} & 85.72{\tiny $\pm$ 1.20} 
                     && 48.84 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Proxy-only-test
                     && 40.64{\tiny $\pm$ 2.89} & 18.58{\tiny $\pm$ 0.36} 
                     & 20.89{\tiny $\pm$ 0.40} & 69.10{\tiny $\pm$ 0.26} 
                     & 70.40{\tiny $\pm$ 1.54} & 10.86{\tiny $\pm$ 0.30} & 81.69{\tiny $\pm$ 1.99} & 85.38{\tiny $\pm$ 1.07} 
                     && 49.69 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Singleton-max        
                     && 29.10 & 19.77
                     & 21.10 & 50.01
                     & 50.00 & 11.83 & 47.97 & 50.00 
                     && 34.97 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13} 
        & Singleton-mean 
                     && 25.14 & 18.75 
                     & 20.68 & 50.00 
                     & 50.00 & 10.84 & 45.83 & 50.00 
                     && 33.91 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13} 
        & Social-Learning-32
                     && 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 0s.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     && 00.00 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Social-Learning-80
                     && 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 0s.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     && 00.00 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Uniform-budget
                     && 32.94{\tiny $\pm$ 00.00} & 18.93{\tiny $\pm$ 00.00} 
                     & 20.70{\tiny $\pm$ 00.00} & 45.69{\tiny $\pm$ 00.00} 
                     & 33.65{\tiny $\pm$ 00.00} & 12.00{\tiny $\pm$ 00.00} & 67.53{\tiny $\pm$ 00.00} & 63.20{\tiny $\pm$ 00.00} 
                     && 36.83 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Random-budget
                     && 32.82{\tiny $\pm$ 0.82} & 19.09{\tiny $\pm$ 0.02} 
                     & 20.75{\tiny $\pm$ 0.07} & 46.11{\tiny $\pm$ 1.24} 
                     & 34.68{\tiny $\pm$ 0.59} & 12.20{\tiny $\pm$ 0.21} & 67.16{\tiny $\pm$ 0.85} & 65.37{\tiny $\pm$ 0.80} 
                     && 37.27 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & $\infty$-budget
                     && 43.26 & 21.70
                     & 20.00 & 62.53
                     & 77.20 & 13.23 & 85.57 & 91.4
                     && 51.37 \\
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Ours
                     && 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     && 00.00 \\ \hline\hline
        \multirow{6}{*}{\begin{sideways}Generates\end{sideways}} 
        % & Zero-shot 
        %              && 00.00 & 00.00 & 00.00 
        %              & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 && 00.00\\
        %              \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        % & Proxy-only 
        %              && 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
        %              & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
        %              & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
        %              && 00.00{\tiny $\pm$ 00.00} \\ 
        %              \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Singleton-max         
                     && 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     && 00.00 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Social Learning
                     && 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     && 00.00 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Uniform-budget
                     && 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     && 00.00 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Random-budget
                     && 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     && 00.00 \\ 
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & $\infty$-budget
                     && 00.00 & 00.00 & 00.00 
                     & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 && 00.00\\
                     \cmidrule{2-2} \cmidrule{4-11} \cmidrule{13-13}  
        & Ours
                     && 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} & 00.00{\tiny $\pm$ 00.00} 
                     && 00.00 \\ 
    \thickhline
    \end{tabular}}
    \caption{Caption. For algorithms using ICL (except Zero-shot), the number of ICEs fed into LLM is 32 for all datasets. The default is 4 clients NonIID}
    \label{tab:my_label}
\end{table*}

==> section/99_limitation.tex <==


\newpage
\myparagraph{Limitations.}
This research addresses in-context learning with datasets distributed among clients with non-iid data. One limitation of this study can be described as follows: (1) Proxy dataset: In practice, some datasets might lack a proxy dataset on the server side, posing a challenge for the proposed algorithm. 
(2) The research assumes the use of a pre-trained off-the-shelf retriever. However, this retriever may fail if there is a significant difference between the target task domain and the pre-trained domain. 
This issue can be mitigated by employing the contrastive training mechanism suggested in federated learning research~\cite{seo2024relaxed}, as one effective approach for training retrievers is utilizing contrastive loss.

\myparagraph{Ethical statement.}
As outlined in the main manuscript, utilizing distributed knowledge raises privacy concerns. We address this by employing a paraphrasing technique developed and frequently used in federated learning with pre-trained generative models, although it has not been thoroughly explored. 
We will make every effort to eliminate privacy concerns and implement all possible measures to prevent privacy information leakage when applying the paraphrasing method to the best of our ability.
